CLMSM: A Multi-Task Learning Framework for Pre-training on Procedural Text

In this paper, we propose CLMSM, a domain-specific, continual pre-training framework, that learns from a large set of procedural recipes. CLMSM uses a Multi-Task Learning Framework to optimize two objectives - a) Contrastive Learning using hard triplets to learn fine-grained differences across entities in the procedures, and b) a novel Mask-Step Modelling objective to learn step-wise context of a procedure. We test the performance of CLMSM on the downstream tasks of tracking entities and aligning actions between two procedures on three datasets, one of which is an open-domain dataset not conforming with the pre-training dataset. We show that CLMSM not only outperforms baselines on recipes (in-domain) but is also able to generalize to open-domain procedural NLP tasks.

==> Sections/Analysis.tex <==
%\section{Analysis and Discussion}
%\label{sec:analysis}
%\noteng{what is the main thing you are trying to tell, express that in 5-6 sentences and push the rest to appendix. }



%\clsm\ is pre-trained on the domain of recipes, and hence, it is expected to perform well on in-domain downstream task datasets such as NPN-Cooking and ARA. However, we are also able to show considerable improvement in the open-domain ProPara Dataset using \clsm.

% \iffalse

\section{Why \clsm\ works}
\label{whyclmsm}

\subsection{Advantages of the proposed pre-training objectives}
We analyze the utility of our proposed pre-training objectives by answering the following research questions - (a) \textit{\textbf{Does masking step(s) help?}} - We check the advantage of MSM by masking random spans instead of step(s), and represent the model as $\clsm_{RANDOMSPAN}$. For a fair comparison, we mask the same percentage of tokens when masking random spans and when masking step(s). We observe that the test accuracy in NPN-Cooking and average category score in ProPara are reduced by $1.8\%$ and $7.65\%$ respectively, suggesting that the masking step(s) signal is vital to enhancing downstream task performance. (b) \textit{\textbf{Utility of using Hard Triplets in CL}} -
We use easy triplets instead of hard triplets to see if fine-grained differences between anchor and negative procedures are indeed helpful. For sampling easy triplets, the positive recipe name is similar to the anchor recipe name (definition of ``similar'' is mentioned in Section \ref{pretr_details}), and the negative recipe name is not similar to the anchor recipe name. We observe that the test accuracy in NPN-Cooking and average category score in ProPara are reduced by $1.46\%$ and $5.46\%$ respectively, suggesting that, the choice of using hard triplets is indeed helpful for procedural reasoning.

% \fi

% \subsection{Reason behind domain generalizability}
%We also analyze the predictions of \clsm\ in the open-domain scenario. 


==> Sections/OLD_expts_and_results.tex <==
\section{Experiments and Results}
\label{sec: expts_results}

We assess the performance of \clsm\ by evaluating its performance on downstream tasks vis-a-vis baselines on the datasets described in Section \ref{downstream} and list inferences that can be drawn. This is followed by an ablation analysis of \clsm. For all the tasks we consider
as a baseline \clsmCascBold\ as a variation of \clsm\ that uses a cascaded framework (CASC.) instead of MTL, i.e, \abhi{it performs CL followed by MSM}, instead of optimizing both the objectives simultaneously. %\abhi{add diagram in appendix maybe}

%\subsection{Baselines}
%Here, we discuss the baselines used for comparison with \clsm\ for the downstream tasks of tracking entities and aligning actions. We first discuss a variation in the \clsm\ framework used as a baseline, followed by task-specific baselines.

%\subsubsection{Variation in \clsm\ as baseline}

\

\subsection{Downstream Task 1:  Tracking Entities}
\label{track_ents_tasks}

% We fine-tune and evaluate on $1$ domain-specific and $1$ open-domain entity tracking task.
% \abhi{common baselines, then specific ones}

We first discuss the baselines (common as well as dataset-specific) for the NPN-Cooking and ProPara Datasets followed by the results. 
An elaborate explanation of baselines from prior works is presented \emph{\textbf{in Section \ref{appendix:baselines1} of Appendix.}}  

\noindent \textbf{Common Baselines: }The following baselines have been shown to work satisfactorily well for both in-domain and open-domain downstream tasks in prior works, and are hence common for the NPN-Cooking and ProPara Datasets - \textbf{KG-MRC} \cite{KGMRC}, \textbf{DYNAPRO} \cite{dynapro}, and $\mathbf{RECIPES_{RB}}$ (model obtained after pre-training RoBERTa-BASE on the corpus of recipes using MLM,  fine-tuned as described in Section \ref{track_ents_tasks}.). 

\noindent \textbf{Dataset-specific Baselines (NPN-Cooking): } We use the Neural Process Network Model (\textbf{NPN-Model}) \cite{npn_paper} as a baseline. 
% Both methods are being evaluated for their ability to track entities and changes in a procedural text. }

\noindent \textbf{Dataset-specific Baselines (ProPara): }We use the following dataset-specific baselines - a \textbf{rule-based} method called \textbf{ProComp} \cite{rule-based-procomp}, a \textbf{feature-based} method \cite{propara-paper} using Logistic Regression and a CRF model, \textbf{ProLocal} \cite{propara-paper}, \textbf{ProGlobal} \cite{propara-paper}, \textbf{EntNet} \cite{entnet}, \textbf{QRN} \cite{QRN}, \textbf{NCET} \cite{ncet}, and $\mathbf{RECIPES_{RL}}$ (which is similar to $\mathbf{RECIPES_{RB}}$, except that, RoBERTa-LARGE is used instead of RoBERTa-BASE.). 
%\pg{Last few citations are for the CRF method / something else -- not clear from this paragraph.} \abhi{these baselines are from TSLM paper, which mentions these citations}

\noindent\textbf{Results (NPN-Cooking): }
\abhi{We compare the previously discussed baselines with} $\clsm_{RB}$ (pre-trained \clsm\ model with RoBERTa-BASE encoder). Similarly, we represent the \clsmCascBold\ baseline as $\clsm_{CASC, RB}$. The results are shown in Table \ref{tab:npn-baselines}. We can infer that - (1) NPN-Model and KG-MRC give poor results due to the lack of an end-to-end neural architecture and prior knowledge through pre-trained models. (2) DYNAPRO uses an end-to-end neural architecture and a pre-trained language model to get entity representations, and performs better than NPN-Model and KG-MRC. (3) $RECIPES_{RB}$ performs better than DYNAPRO due to domain-specific pre-training \abhi{(4) $\clsm_{CASC}$ is the best baseline, suggesting %that the additional pre-training done using \clsmCasc\ improves results, as 
CL when followed by MSM improves procedural context understanding (5) $\clsm_{RB}$ gives the best test accuracy among all models, 
suggesting that, MTL performs better than optimizing the objectives sequentially. } %However,  masking multiple steps together sometimes impedes fine-grained learning (for inferring the exact step where the entity location changes), resulting in a slightly inferior performance at M=2. %(6) Also, masking $2$ steps instead of $1$ step does not help \clsm\, and gives a negligible boost to the performance of \clsmCasc, which is because predicting masked tokens of two random steps is harder than predicting that of a random step. \noteng{so what}
% \noteng{I think we need to discuss this}
\begin{table}[!htb]
\centering
\begin{tabular}{l|c}
\hline
 & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}TEST\\ ACCURACY\end{tabular}}} \\ \hline
NPN-Model    & 51.3           \\
KG-MRC       & 51.6           \\
DYNAPRO      & 62.9           \\
$\text{RECIPES}_{\text{RB}}$ & 63.8          \\
% $\clsm_{CASC., RB, M=1}$  & 63.92 \\ 
% $\clsm_{CASC., RB, M=2}$  & 63.99 \\ \hline
$\clsm_{CASC., RB}$  & 63.99 \\ \hline
% $\clsm_{RB, M=1}$  & \textbf{64.24} \\ 
% $\clsm_{RB, M=2}$  & 62.89 \\ \hline
$\clsm_{RB}$  & \textbf{64.62} \\ \hline
\end{tabular}
\caption{Results when fine-tuned on the NPN-Cooking Dataset - Baselines vs. \clsm \noteng{WHy is RL not mentioned here}}
\label{tab:npn-baselines}
\end{table}



\noindent \textbf{Results (ProPara): } \noteng{provide table number which you are }We compare the previously discussed baselines with $\clsm_{RB}$ on the ProPara Dataset \abhi{in Table \ref{tab:propara-baselines}}.%, having RoBERTa-BASE encoder architecture. 
% Note that here, the bidirectional transformer in \clsm\ is initialized using RoBERTa-BASE and RoBERTa-LARGE architectures, similar to \newcite{TSLM}. 
We observe that - (1) Rule-based and Feature-based baselines perform poorly, as they cannot generalize well to the unseen vocabulary in the test set (2) ProLocal performs slightly better, but the improvement in the Cat. 3 Score (corresponding to the location of an entity) is negligible. This can be due to ProLocal making local predictions, thus having poor global consistency. (3) ProGlobal shows a considerable improvement in the Cat. 3 Score, as it attends across the entire procedure, thus having better global consistency (4) EntNet and QRN perform poorly, as they both follow very simple recurrent update mechanisms, that are not complex enough to understand procedures effectively. (5) KG-MRC performs better than almost all previously discussed baselines, as it builds a dynamic Knowledge Graph of entities and states, which then becomes a structured input to the MRC, making it easier to figure out the entity's state. (6) NCET and DYNAPRO achieve high evaluation metrics, as NCET uses extra action/verb information, while DYNAPRO uses an open-domain pre-trained language model in its framework.
% , which matches the open-domain nature of the downstream dataset. 
This is the reason behind these models performing better than $RECIPES_{RB}$, which is pre-trained on recipes. DYNAPRO especially gives a high Cat. 3 Score due to an additional Bi-LSTM that smoothens predicted locations across steps, while adding additional fine-tuning overhead.
\noteng{But DYNAPRO has a very good CAT3 score, why} 
\abhi{(7) $\clsm_{RB}$ outperforms $5$ baselines on all $3$ metrics. } \noteng{not true, }
% Similar to the NPN-Cooking Dataset, masking two steps deteriorates performance for \clsm\ and \clsmCasc. 
Also, \clsmCasc\ performs inferior to \clsm\ (except for the Cat. 3 Score)
(8) We also experiment with \clsm\  with an encoder having RoBERTa-LARGE architecture
 - \abhi{$\clsm_{RL}$ on the ProPara Dataset. The results are shown in Table \ref{tab:propara-baselines}. We can see that $\clsm_{RL}$ performs the best w.r.t Cat. 1 and Cat. 2 Scores. The dip in the Cat. 3 Score compared to $\mathbf{RECIPES_{RL}}$ is negligible ($0.08\%$), even though  \clsm\ is pre-trained on domain-specific corpora (unlike the domain-specific ProPara Dataset). $\clsm_{RL}$ gives an improvement of $3.33\%$ over $RECIPES_{RL}$ in terms of average category score.} %(9) Also, masking two steps when using a RoBERTa-LARGE encoder improves performance compared to masking one step, as a larger encoder is better equipped at predicting a larger number of tokens.
 % Also, $\clsm_{MTL-PP}$ performs better than $6$ baselines (including RoBERTa-BASE), even though a smaller RoBERTa-BASE encoder architecture is used in this case.
% Especially, all the $3$ \clsm\ variants perform better than all baselines w.r.t Cat. 2 Score, which requires predicting the step when an entity is created, moved, or destroyed. This shows that the \clsm\ has good procedural comprehension when fine-tuned on an open-domain procedural downstream task, even though it has been pre-trained on domain-specific recipe corpus.

\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|ccc}
\hline
 &
  \begin{tabular}[c]{@{}c@{}}\textbf{TEST}\\ \textbf{CAT. 1}\\ \textbf{SCORE}\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}\textbf{TEST}\\ \textbf{CAT. 2}\\ \textbf{SCORE}\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}\textbf{TEST}\\ \textbf{CAT. 3}\\ \textbf{SCORE}\end{tabular} \\ \hline
Rule-based    & 57.14         & 20.33          & 2.4            \\
Feature-based & 58.64         & 20.82          & 9.66           \\
ProLocal      & 62.7          & 30.5           & 10.4           \\
ProGlobal     & 63            & 36.4           & 35.9           \\
EntNet        & 51.6          & 18.8           & 7.8            \\
QRN           & 52.4          & 15.5           & 10.9           \\
KG-MRC           & 62.9 & 40.0 & 38.2           \\
NCET & 73.7 & 47.1 & 41.0 \\
DYNAPRO & 72.4 & 49.3 & \textbf{44.5} \\
$\text{RECIPES}_{\text{RB}}$  & 71.33         & 34.11          & 30.86          \\ 
$\text{RECIPES}_{\text{RL}}$  & 74.58 &	47.53 &	38.37          \\
% $\clsm_{CASC., RB, M=1}$ &   67.94	& 36.85	& 35.94 \\
% $\clsm_{CASC., RB, M=2}$       & 65.54 &	32.4 &	32.9  \\
$\clsm_{CASC., RB}$ &   67.94	& 36.85	& 35.94 \\
\hline
% $\clsm_{RB, M=1}$       & 72.6 & 38.54          & 35.24          \\
% $\clsm_{RB, M=2}$       & 69.21 & 38.39          & 34.35          \\
$\clsm_{RB}$       & 69.92 & 39.35          & 33.89          \\

% $\clsm_{CAT2}$       & 70.9          & \textbf{39.52} & 33.76          \\
% $\clsm_{CAT3}$       & 69.77         & 37.05          & \textbf{38.02} \\ 

 
% $\clsm_{RL, M=1}$       & 75.14	& 47.96 &	36.84     \\
% $\clsm_{RL, M=2}$       & \textbf{77.26}	& \textbf{54.86} &	38.34     \\
$\clsm_{RL}$       & \textbf{77.26}	& \textbf{54.86} &	38.34     \\
% $\clsm_{L-CAT2}$       & 70.9          & \textbf{39.52} & 33.76          \\
% $\clsm_{L-CAT3}$       & 69.77         & 37.05          & \textbf{38.02} \\ 
\hline
\end{tabular}%
}
\caption{Results when fine-tuned on the ProPara Dataset - Baselines vs. \clsm}
\label{tab:propara-baselines}
\end{table}

\subsection{Case Study}
Table \ref{tab:propara_preds} shows the ground truth annotations and the predictions of $\clsm_{RL}$ and $RECIPES_{RL}$ on a procedure from the ProPara Dataset that describes the process of the growth of a tree. We have chosen this sample, as the ground truth annotations are not very varied, making it easier to analyze. We can infer that - (1) $RECIPES_{RL}$ tends to predict a location span in the same step as the entity (while the actual location might be present in some other step), which suggests that $RECIPES_{RL}$ is not able to focus on long-range contexts across steps (2) \clsm\ is able to better understand long-range contexts. E.g. in the case of the entities ``seedling'' and ``root system'', \clsm\ correctly predicts the location corresponding to the ground truth ``ground" for most steps (unlike $RECIPES_{RL}$), even though ``ground" is mentioned only once in the first step of the procedure. This is because \clsm\ learns local as well as global procedural contexts during pre-training. Hence, \clsm\ performs better than $RECIPES_{RL}$ for tracking entities whose locations are implicit in nature, i.e., the location at the current step requires retention of knowledge from a step far in the past.

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

A quantitative analysis of the type of predictions made by \clsm\ and $RECIPES_{RL}$ on ProPara is discussed \emph{\textbf{in Section \ref{appendix:case_study} of Appendix.}} %We infer that \clsm\ performs better than $RECIPES_{RL}$ in cases when the location of the entity in a step is known, as well as when it is unknown.



\subsection{Downstream Task 2: Aligning Actions}
%\noindent \textbf{Dataset 3: ARA: }
\abhi{We compare $\clsm_{BERT}$ %and $\clsm_{BERT, M=2}$ (architecture of the bidirectional encoder being BERT-BASE-UNCASED)
with the baselines $\mathbf{RECIPES_{BERT}}$  %which is BERT-BASE-UNCASED pre-trained on the corpus of recipes using MLM, 
and \clsmCasc\ variant $\clsm_{CASC., BERT}$. 
%and $\clsm_{CASC., BERT, M=2}$. %\abhi{ADD BASELINES}

\noindent \textbf{Results (ARA): }
We can see from Table \ref{tab:ara-baselines} that $\clsm_{BERT}$ performs the best, showing an improvement of about $4.28\%$ over the baseline $\mathbf{RECIPES_{BERT}}$. Even here, \clsm\ variants outperform \clsmCasc\ variants.} %However, masking two steps instead of one step in \clsm\ here improves results, as aligning actions between recipes is better enabled if there is a understanding of more than one step. 
% \noteng{Again reasoning is needed... due to the nature of the task? where we are not probling inside a step but consider the entire step together}
\abhi{The lesser the distance between ground truth and predicted word tokens\footnote{Distance between two tokens is $0$ if they are the same, and $1$ more than the number of tokens in between, considering the procedure as a paragraph otherwise}, the better the model. We observe that $\clsm_{BERT}$ gives a better mean distance of $12.72$, compared to $\mathbf{RECIPES_{BERT}}$, which gives a mean distance of $13.31$.}

\begin{table}[!htb]
\centering
\begin{tabular}{l|c}
\hline
 & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}TEST\\ ACCURACY\end{tabular}}} \\ \hline
$\text{RECIPES}_{\text{BERT}}$ & 64.22          \\ 
% $\clsm_{CASC., BERT, M=1}$ & 55.96 \\
% $\clsm_{CASC., BERT, M=2}$ & 46.79
%  \\
$\clsm_{CASC., BERT}$ & 55.96 \\
\hline
% $\clsm_{BERT, M=1}$  & 57.8 \\ 
% $\clsm_{BERT, M=2}$  & \textbf{66.97} \\ \hline
$\clsm_{BERT}$  & \textbf{66.97} \\ \hline
\end{tabular}
\caption{Results when fine-tuned on the ARA Dataset - Baselines vs. \clsm}
\label{tab:ara-baselines}
\end{table}

% Also, $7$ out of the $12$ $\clsm_{MTL}$ variants perform better than \textbf{BERT-BASE-UNCASED}.


\subsection{Ablation Experiments}
\begin{table}[!htb]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|ccc}
\hline
 &
  \begin{tabular}[c]{@{}c@{}}\textbf{TEST}\\\textbf{CAT. 1}\\ \textbf{SCORE}\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}\textbf{TEST}\\\textbf{CAT. 2}\\ \textbf{SCORE}\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}\textbf{TEST}\\\textbf{CAT. 3}\\ \textbf{SCORE}\end{tabular} \\ \hline
$\clsm_{RB}(CL)$   & 67.8          & 35.62          & 33.61          \\
% $\clsm_{RB, M=1}(MSM)$ & 70.9          & 37.61          & \textbf{34.05}          \\
% $\clsm_{RB, M=2}(MSM)$ & 67.09         & 36.83          & 34.03          \\ \hline
$\clsm_{RB}(MSM)$ & 67.09         & 36.83          & \textbf{34.03}          \\ \hline
% $\clsm_{RB, M=1}$            & \textbf{72.6} & \textbf{38.54} & \textbf{35.24} \\
% $\clsm_{RB, M=2}$            & 69.21         & 38.39          & 34.35          \\ \hline
$\clsm_{RB}$            & \textbf{69.92}         & \textbf{39.35}          & 33.89          \\ \hline
\end{tabular}%
}
\caption{Ablation Analysis of \clsm\ on the ProPara Dataset}
\label{tab:ablation}
\end{table}

\begin{table*}[!htb]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|cccc|cccc|cccc}
\hline
 &
  \multicolumn{4}{c|}{Ground Truth} &
  \multicolumn{4}{c|}{$\clsm_{RL}$} &
  \multicolumn{4}{c}{$RECIPES_{RL}$} \\ \hline
Procedure &
  seedling &
  \begin{tabular}[c]{@{}c@{}}root\\ system\end{tabular} &
  tree &
  \begin{tabular}[c]{@{}c@{}}material\\ for new\\ growth\end{tabular} &
  seedling &
  \begin{tabular}[c]{@{}c@{}}root\\ system\end{tabular} &
  tree &
  \begin{tabular}[c]{@{}c@{}}material\\ for new\\ growth\end{tabular} &
  seedling &
  \begin{tabular}[c]{@{}c@{}}root\\ system\end{tabular} &
  tree &
  \begin{tabular}[c]{@{}c@{}}material\\ for new\\ growth\end{tabular} \\ \hline
(Before the process starts) &
  ground &
  - &
  - &
  - &
  {\color[HTML]{FE0000} -} &
  {\color[HTML]{009901} -} &
  {\color[HTML]{009901} -} &
  {\color[HTML]{009901} -} &
  {\color[HTML]{FE0000} -} &
  {\color[HTML]{009901} -} &
  {\color[HTML]{009901} -} &
  {\color[HTML]{009901} -} \\
1. A seedling is grown in the ground. &
  ground &
  - &
  - &
  - &
  {\color[HTML]{009901} ground} &
  {\color[HTML]{009901} -} &
  {\color[HTML]{009901} -} &
  {\color[HTML]{009901} -} &
  {\color[HTML]{009901} ground} &
  {\color[HTML]{009901} -} &
  {\color[HTML]{009901} -} &
  {\color[HTML]{009901} -} \\
\begin{tabular}[c]{@{}l@{}}2. The seedling grows bigger, and forms\\  its root system.\end{tabular} &
  ground &
  ground &
  - &
  - &
  {\color[HTML]{009901} ground} &
  {\color[HTML]{009901} ground} &
  {\color[HTML]{009901} -} &
  {\color[HTML]{009901} -} &
  {\color[HTML]{FE0000} -} &
  {\color[HTML]{FE0000} seed} &
  {\color[HTML]{009901} -} &
  {\color[HTML]{009901} -} \\
\begin{tabular}[c]{@{}l@{}}3. The roots start to gain more nourishment \\ as the tree grows.\end{tabular} &
  ground &
  ground &
  ground &
  - &
  {\color[HTML]{009901} ground} &
  {\color[HTML]{009901} ground} &
  {\color[HTML]{009901} ground} &
  {\color[HTML]{009901} -} &
  {\color[HTML]{FE0000} -} &
  {\color[HTML]{FE0000} tree} &
  {\color[HTML]{009901} ground} &
  {\color[HTML]{009901} -} \\
\begin{tabular}[c]{@{}l@{}}4. The tree starts to attract animals and plants\\  that will grant it more nourishment.\end{tabular} &
  ground &
  ground &
  ground &
  - &
  {\color[HTML]{009901} ground} &
  {\color[HTML]{009901} ground} &
  {\color[HTML]{009901} ground} &
  {\color[HTML]{009901} -} &
  {\color[HTML]{FE0000} -} &
  {\color[HTML]{009901} ground} &
  {\color[HTML]{009901} ground} &
  {\color[HTML]{009901} -} \\
5. The tree matures. &
  ground &
  ground &
  ground &
  - &
  {\color[HTML]{FE0000} -} &
  {\color[HTML]{009901} ground} &
  {\color[HTML]{009901} ground} &
  {\color[HTML]{009901} -} &
  {\color[HTML]{FE0000} -} &
  {\color[HTML]{009901} ground} &
  {\color[HTML]{009901} ground} &
  {\color[HTML]{009901} -} \\
\begin{tabular}[c]{@{}l@{}}6. After a number of years the tree will \\ grow old and die, becoming material \\ for new growth.\end{tabular} &
  ground &
  ground &
  - &
  ground &
  {\color[HTML]{FE0000} -} &
  {\color[HTML]{009901} ground} &
  {\color[HTML]{009901} -} &
  {\color[HTML]{FE0000} tree} &
  {\color[HTML]{FE0000} -} &
  {\color[HTML]{009901} ground} &
  {\color[HTML]{009901} -} &
  {\color[HTML]{FE0000} tree} \\ \hline
\end{tabular}%
}
\caption{Analysis of the ground truth and the predictions of \clsm\ vs. a well-performing baseline on a sample from the ProPara Dataset. \clsm\ is able to predict the ground truth location ``ground" in most steps, even though ``ground" is mentioned only once in the first step}
\label{tab:propara_preds}
\end{table*}

We conducted ablation experiments considering each loss separately, i.e., we use only CL and only MSM as objectives during pre-training. We show results on the ProPara Dataset in Table \ref{tab:ablation} (\clsm\ uses a RoBERTa-BASE (RB) architecture for its bidirectional encoder).
\abhi{We can infer that the combination of CL and MSM ($\clsm_{RB}$) performs better than the models that use only MSM or only CL on the Cat. 1 and Cat. 2 Scores, with an average improvement of $3.78\%$ compared to the best ablation.} This shows that CL and MSM objectives reinforce each other. The results are similar for the other $2$ datasets, as discussed \emph{\textbf{in Section \ref{appendix:ablation} of Appendix}}.%\noteng{Are the results similar for other cases, then please mention that.}
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\noteng{in an odd place}


